geodesiq: a Python package for geometric diabatic-adiabatic optimal state transfer

We introduce the geodesiq Python package, which implements a geometric framework for shaping control pulses that achieve high-fidelity state transfer in multilevel quantum systems. The underlying method combines adiabatic and diabatic control into a single metric, suppressing unwanted excitations while allowing selected diabatic passages. Finding the pulse thereby reduces to solving a single first-order ordinary differential equation. We explain how to use geodesiq and illustrate its use explicitly with Landau-Zener transitions, spin-qubit initialization, adiabatic many-body ground-state preparation, and a diabatic-adiabatic transfer in a four-level system.

==> Extras/notebook_window.tex <==
\begin{tikzpicture}[every node/.style={inner sep=0pt}]
\definecolor{titlebarcol}{RGB}{237,237,237}
\definecolor{toolbarcol}{RGB}{250,250,250}
\definecolor{closebtn}{RGB}{255,95,87}
\definecolor{minbtn}{RGB}{255,189,46}
\definecolor{maxbtn}{RGB}{39,201,63}
\definecolor{incolor}{RGB}{44,62,152}
\definecolor{outcolor}{RGB}{183,28,28}
\definecolor{cellborder}{RGB}{207,207,207}
\definecolor{selectbar}{RGB}{66,133,244}
\definecolor{jkw}{RGB}{0,128,0}
\definecolor{jstr}{RGB}{186,33,33}
\definecolor{jnum}{RGB}{102,102,102}
\definecolor{jfn}{RGB}{0,0,255}
\def\nbkw#1{\textcolor{jkw}{\textbf{#1}}}
\def\nbstr#1{\textcolor{jstr}{#1}}
\def\nbnum#1{\textcolor{jnum}{#1}}
\def\nbfn#1{\textcolor{jfn}{#1}}
\pgfmathsetlengthmacro{\promptw}{1.45cm}
\pgfmathsetlengthmacro{\cellw}{\outputwidth + 10pt}
\pgfmathsetlengthmacro{\winw}{0.3cm + \promptw + \cellw + 0.45cm}
\def\titleh{0.62cm}
\def\toolh{0.45cm}

\foreach \c [count=\i] in {closebtn, minbtn, maxbtn}
    \filldraw[fill=\c, draw=\c!60!black, line width=0.3pt] (0.15cm + \i*0.3cm, -\titleh/2) circle (0.075cm);
\node[font=\fontsize{8}{10}\selectfont, text=black!55] at (\winw/2, -\titleh/2) {\notebookname};

\node[font=\ttfamily\fontsize{7}{8}\selectfont, text=black!45, anchor=west] at (0.45cm, -\titleh-\toolh/2)
    {[+ Code]\quad[Run]\quad[Restart]\quad[Save]};

\node[font=\ttfamily\fontsize{8}{10}\selectfont, text=incolor, anchor=north west] (inlabel)
    at (0.3cm, -\titleh-\toolh-0.35cm) {In\,[1]:};
\node[draw=cellborder, rounded corners=2.5pt, fill=white, align=left, font=\ttfamily\fontsize{8}{10}\selectfont,
      inner sep=5pt, text width=\cellw-10pt, anchor=north west] (incell)
    at (0.3cm + \promptw, -\titleh-\toolh-0.3cm) {\notebookcode};
\draw[selectbar, line width=2.2pt] ([xshift=-0.09cm]incell.north west) -- ([xshift=-0.09cm]incell.south west);

\node[font=\ttfamily\fontsize{8}{10}\selectfont, text=outcolor, anchor=north west] (outlabel)
    at ([yshift=-0.35cm]inlabel.west |- incell.south) {Out[1]:};
\node[draw=cellborder, rounded corners=2.5pt, fill=white, inner sep=5pt, anchor=north west] (outimg)
    at ([yshift=-0.3cm]incell.south west) {\includegraphics[width=\outputwidth]{\outputimage}};

\coordinate (br) at (\winw, 0 |- outimg.south);
\coordinate (br) at ([yshift=-0.3cm]br);
\begin{scope}[on background layer]
    \fill[black!20, rounded corners=6pt] ([xshift=1.2pt, yshift=-1.2pt]0,0) rectangle ([xshift=1.2pt, yshift=-1.2pt]br);
    \begin{scope}
        \clip[rounded corners=6pt] (0,0) rectangle (br);
        \fill[white] (0,0) rectangle (br);
        \fill[titlebarcol] (0,0) rectangle (\winw, -\titleh);
        \fill[toolbarcol] (0,-\titleh) rectangle (\winw, -\titleh-\toolh);
    \end{scope}
    \draw[rounded corners=6pt, draw=black!35, line width=0.5pt] (0,0) rectangle (br);
    \draw[black!15, line width=0.4pt] (0,-\titleh) -- (\winw,-\titleh);
    \draw[black!10, line width=0.4pt] (0,-\titleh-\toolh) -- (\winw,-\titleh-\toolh);
\end{scope}
\end{tikzpicture}%

